Information-Theoretic Generalization Bounds for SGLD via Data-Dependent Estimates

In this work, we improve upon the stepwise analysis of noisy iterative learning algorithms initiated by Pensia, Jog, and Loh (2018) and recently extended by Bu, Zou, and Veeravalli (2019). Our main contributions are significantly improved mutual information bounds for Stochastic Gradient Langevin Dynamics via data-dependent estimates. Our approach is based on the variational characterization of mutual information and the use of data-dependent priors that forecast the mini-batch gradient based on a subset of the training samples. Our approach is broadly applicable within the information-theoretic framework of Russo and Zou (2015) and Xu and Raginsky (2017). Our bound can be tied to a measure of flatness of the empirical risk surface. As compared with other bounds that depend on the squared norms of gradients, empirical investigations show that the terms in our bounds are orders of magnitude smaller.

==> arxiv final/acknowledgements.tex <==
JN is supported by an NSERC Vanier Canada Graduate Scholarship, and by the Vector Institute.
MH was supported by a MITACS Accelerate Fellowship with Element AI.
DMR is supported by an NSERC Discovery Grant and an Ontario Early Researcher Award.
This research was carried out in part while GKD and DMR were visiting the Simons Institute for the Theory of Computing.


==> arxiv final/authors.tex <==
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\author{
	Jeffrey Negrea\thanks{Equal contribution authors, order of names was determined randomly.}\\
  University of Toronto,\\
	Vector Institute \\
	\And
	Mahdi Haghifam\samethanks\\
	University of Toronto, \\
	Element AI \\
	\And
	Gintare Karolina Dziugaite \\
	Element AI \\
	\And
	Ashish Khisti \\
	University of Toronto \\
	\And
	Daniel M. Roy \\
	University of Toronto,\\
	Vector Institute
}


==> arxiv final/defs.tex <==
%

\def\[#1\]{\begin{align}#1\end{align}}
\def\*[#1\]{\begin{align*}#1\end{align*}}

\newcommand{\defas}{\vcentcolon=}  %
%

%
\newcommand{\minf}[1]{I(#1)}

%
\newcommand{\cPr}[2]{\Pr^{#1}[#2]}

%
\newcommand{\st}{\,:\,}
\newcommand{\ip}[2]{\langle #1,#2\rangle}
\newcommand{\uniform}[1]{\mathcal{U}[#1]}

\newcommand{\pmean}{\bar w}
\newcommand{\parspace}{\mathcal{W}}
\newcommand{\Dist}{\mathcal D}
\newcommand{\dataspace}{\mathcal Z}
\newcommand\optparen[1]{\ifthenelse{\equal{#1}{}}{}{(#1)}}
\newcommand{\RiskChar}{R}
\newcommand{\Risk}[2]{\RiskChar_{#1}\optparen{#2}}
\newcommand{\EmpRisk}[2]{\hat \RiskChar_{#1}\optparen{#2}}
\newcommand{\SurRisk}[2]{\tilde \RiskChar_{#1}\optparen{#2}}
\newcommand{\SurEmpRisk}[2]{\tilde \RiskChar_{#1}\optparen{#2}}
\newcommand{\EmpDist}{\hat\Dist}
\newcommand{\Lmax}{L_{\text{max}}}

\newcommand{\set}[2][]{#1\{#2 #1\}}
\newcommand{\brackets}[2][]{#1[#2 #1]}
\newcommand{\parens}[2][]{#1(#2 #1)}

%
\newcommand{\dist}{\ \sim\ }
\newcommand{\given}{\mid}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}

\newcommand{\Gibbs}{\mathcal{G}}

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\BorelSets}{\mathcal{B}}
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\Ints}{\mathbb{Z}}
\newcommand{\NNInts}{\Ints_+}
\newcommand{\NNExtInts}{\overline{\Ints}_+}
\newcommand{\Cantor}{\2^\mathbb{N}}
\newcommand{\NNReals}{\Reals_+}

\newcommand{\as}{\textrm{a.s.}}

\newcommand{\epi}{\textrm{epi}}
\newcommand{\intr}{\textrm{int}}
\newcommand{\conv}{\textrm{conv}}
\newcommand{\cone}{\textrm{cone}}
\newcommand{\aff}{\textrm{aff}}
\newcommand{\dom}{\textrm{dom}}
\newcommand{\cl}{\textrm{cl}}
\newcommand{\ri}{\textrm{ri}}
\newcommand{\grad}{\nabla}
\newcommand{\imp}{\Rightarrow}
\newcommand{\downto}{\!\downarrow\!}
\newcommand{\upto}{\!\uparrow\!}

%
\newcommand{\ind}{\mathrel{\perp\mkern-9mu\perp}}
%
%

\newcommand{\AND}{\wedge}
\newcommand{\OR}{\vee}
\newcommand{\NOT}{\neg}

\newcommand{\dee}{\mathrm{d}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator*{\newlim}{\mathrm{lim}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmin}{\mathrm{min}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmax}{\mathrm{max}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newinf}{\mathrm{inf}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newsup}{\mathrm{sup}\vphantom{\mathrm{infsup}}}
\renewcommand{\lim}{\newlim}
\renewcommand{\min}{\newmin}
\renewcommand{\max}{\newmax}
\renewcommand{\inf}{\newinf}
\renewcommand{\sup}{\newsup}

%
\newcommand{\PowerSet}{\mathcal{P}}

\newcommand{\Measures}{\mathcal{M}}
\newcommand{\ProbMeasures}[1]{\mathcal{M}_1(#1)}

\renewcommand{\Pr}{\mathbb{P}}
\def\EE{\mathbb{E}}
\DeclareMathOperator*{\var}{var}

%
\newcommand{\defn}[1]{\textbf{#1}}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}

\def\bone{\mathbf{1}}
\def\Ind{\bone}

\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}

\DeclareMathOperator*{\Beta}{Beta}
\DeclareMathOperator*{\Bernoull}{Bernoulli}
\DeclareMathOperator*{\PP}{PP}
\DeclareMathOperator*{\Poisson}{Poisson}
\newcommand{\Uniform}{\textrm U (0,1)}

\newcommand{\equaldist}{\overset{d}{=}}
\newcommand{\inv}{^{-1}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\event}[1]{\left \lbrace #1 \right \rbrace}
\newcommand{\tuple}[1]{\langle #1 \rangle}


\newcommand{\bspace}{\Omega}
\newcommand{\bsa}{\mathcal A}
\newcommand{\borelspace}{(\bspace,\bsa)}


\newcommand{\card}[1]{\##1}
%
\newcommand{\iid}{i.i.d.}




\newcommand{\Qsnn}{Q_{\mathrm{SNN}}}
\newcommand{\SigmaSNN}{\Sigma_{\mathrm{SNN}}}

\newcommand{\Sym}{\mathbb{S}}

\newcommand{\KLname}{\mathrm{KL}}
\newcommand{\HH}{\mathcal H}
\newcommand{\KL}[2]{\KLname(#1 \,\|\,#2)}
\newcommand{\klbin}[2]{\mathcal{kl}(#1||#2)}

\newcommand{\BIGKLBOUND}[2]{\KLname^{-1}\biggl(#1 \biggl\lvert#2\biggr)}
\newcommand{\KLBOUND}[2]{\KLname^{-1}(#1|#2)}
%

\newcommand{\PACBayes}{PAC-Bayes}
\newcommand{\REB}{B_{\mathrm{RE}}}
\newcommand{\PosReals}{\Reals_{+}}
\newcommand{\PACBOUND}{B_{\mathrm{PAC}}}
\newcommand{\QUADBOUND}{\bar B_{\mathrm{PAC}}}
\newcommand{\NEWTON}{\mathrm{N}}

\newcommand{\diag}{\mathrm{diag}}

\newcommand{\Normal}{\mathcal N}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\Bernoulli}[1]{\mathcal B(#1)}

\newcommand{\EEE}[1]{\underset{#1}{\EE}}
\newcommand{\PPr}[1]{\underset{#1}{\Pr}}
\newcommand{\Var}{\text{Var}}
\newcommand{\VVar}[1]{\underset{#1}{\Var}}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\CCov}[1]{\underset{#1}{\Cov}}


\newcommand{\XX}{\Reals^{\idim}}
%
\newcommand{\YY}{K}

\newcommand{\ce}{e}
\newcommand{\ece}{\hat \ce}
\newcommand{\bece}{\tilde \ce}

\newcommand{\loss}{\ell}
%
\newcommand{\emploss}{\hat\loss}
\newcommand{\surloss}{\breve\loss}
\newcommand{\surce}{\breve\ce}

\newcommand{\VC}{\mathrm{VCdim}}
\newcommand{\idim}{k}
\newcommand{\pdim}{d}
%

\newenvironment{nouppercase}{%
  \let\uppercase\relax%
  \renewcommand{\uppercasenonmath}[1]{}}{}
  
%
\newcommand{\hypothesisclass}{\mathcal{H}}
\newcommand{\hypclassn}[1]{\mathcal{H}_{#1}}
\newcommand{\datadist}{\mu}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\reals}{\mathbb{R}}
%
\newcommand{\trainset}{S}
\newcommand{\nnclass}{\mathcal{N}}
%

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\id}[1]{\mathbb{I}_{#1}}
\newcommand{\cost}{\text{B}}
\newcommand{\Alog}{\text{A}_{\surloss}}
\newcommand{\wsgd}{w_{\text{SGD} }}
\newcommand{\wsnn}{w_{\text{SNN} }}

\newcommand{\wprior}{w_{\text{prior} }}
\newcommand{\wpost}{w_{\text{post} }}


\newcommand{\Alg}{\mathcal{A}}


\newcommand{\unif}[1]{\text{Unif}(#1)}
\newcommand{\evalat}[1]{\bigg\vert_{#1}}
\newcommand{\bernoulli}{\text{Ber}}
\newcommand{\binomial}{\text{Bin}}

\newcommand{\idx}{\text{idx}}




\newcommand{\lcr}[3]{\left #1 #2 \right #3}
\newcommand{\lcrx}[4][{-1}]{
	\IfEq{#1}{-1}{\left #2 {{{{#3}}}} \right #4}{
   	\IfEq{#1}{0}{#1 {{{{#2}}}} #3}{
	\IfEq{#1}{1}{\bigl #2 {{{{#3}}}} \bigr #4}{
	\IfEq{#1}{2}{\Bigl #2 {{{{#3}}}} \Bigr #4}{
	\IfEq{#1}{3}{\biggl #2 {{{{#3}}}} \biggr #4}{
	\IfEq{#1}{4}{\Biggl #2 {{{{#3}}}} \Biggr #4}{
    \GenericWarning{"4th argument to lcrx must be -1, 0, 1, 2, 3, or 4"}
    }}}}}}}
%
%
%
\newcommand{\ceil}[2][{-1}]{\lcrx[#1] \lceil {#2} \rceil}
%
\newcommand{\inner}[3][{-1}]{\lcrx[#1] \langle {{#2},\ {#3}} \rangle}
%
\newcommand{\rbra}[2][{-1}]{\lcrx[#1] ( {#2} ) }
\newcommand{\sbra}[2][{-1}]{\lcrx[#1] [ {#2} ] }


\newcommand{\rnderiv}[2]{\frac{\text{d} #1}{\text{d} #2}}


==> arxiv final/defs2.tex <==
%
%

\newcommand{\SA}[1]{\cF_{#1}}
\newcommand{\cEE}[1]{\EE^{#1}}
\newcommand{\ww}{W}
%
\newcommand{\bgrad}[2]{\nabla \SurEmpRisk{#1}{#2}}
\newcommand{\rgrad}[1]{\nabla \SurRisk{\Dist}{#1}}

\newcommand{\conditional}[1]{#1_{t|}}
\newcommand{\conditionalt}[2]{#1_{#2|}}
%
\newcommand{\conditionalback}[1]{#1_{|T}}

\newcommand{\RS}{U}


\newcommand\eqdist{\mathrel{\overset{\smash{\makebox[0pt]{\mbox{\normalfont\tiny d}}}}{=}}}
%
\newcommand{\indep}{\mathrel{\perp\mkern-9mu\perp}}

\newcommand{\sloss}{\tilde{\ell}}
\newcommand{\sEmpRisk}{\hat{F}}
%
\newcommand{\dminf}[2]{I^{#1} (#2)}
\newcommand{\cVVar}[2]{\underset{#1}{\text{Var}^{#2}}}


==> arxiv final/headers.tex <==
%

\usepackage{amsmath,amsthm,wrapfig}
	\usepackage[utf8]{inputenc} 
\usepackage{amsmath, amssymb,bm, cases, mathtools, thmtools}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathrsfs} 
%
\usepackage{caption}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
%

\usepackage[%
    minnames=1,maxnames=99,maxcitenames=3,
    style=numeric,%
    sortcites=true,
    doi=false,url=false,
    giveninits=true,
    hyperref,natbib,backend=biber]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
\bibliography{biblio}
%
%


\usepackage[T1]{fontenc}
\usepackage{inconsolata}
\usepackage{mathptmx}

%
%

\usepackage{listings} %

\usepackage{enumitem}
\usepackage{booktabs}       %
%
\usepackage{nicefrac}       %

%
%
%

\usepackage{lineno}
\usepackage{bbm}

%
\usepackage{caption}
\usepackage{subcaption}


\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
%
\usepackage{datetime}

%
%
%

\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
\newcommand{\eurom}{\EuRoman}

%
%


%
\usepackage[capitalize]{cleveref}

%
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{theorem}{Theorem}{Theorems}

%
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother


%
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,qed=$\triangleleft$,sibling=theorem,name=Remark]{remark}
%

%
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%

%
%

\usepackage{xparse}
\usepackage{xstring}

